Efficiency Matters: Speeding Up Automated Testing with GUI Rendering Inference

Due to the importance of Android app quality assurance, many automated GUI testing tools have been developed. Although the test algorithms have been improved, the impact of GUI rendering has been overlooked. On the one hand, setting a long waiting time to execute events on fully rendered GUIs slows down the testing process. On the other hand, setting a short waiting time will cause the events to execute on partially rendered GUIs, which negatively affects the testing effectiveness. An optimal waiting time should strike a balance between effectiveness and efficiency. We propose AdaT, a lightweight image-based approach to dynamically adjust the inter-event time based on GUI rendering state. Given the real-time streaming on the GUI, AdaT presents a deep learning model to infer the rendering state, and synchronizes with the testing tool to schedule the next event when the GUI is fully rendered. The evaluations demonstrate the accuracy, efficiency, and effectiveness of our approach. We also integrate our approach with the existing automated testing tool to demonstrate the usefulness of AdaT in covering more activities and executing more events on fully rendered GUIs.

==> background.tex <==
\section{Background}
This section introduces the background of the mature Android testing tools, and the configurations we used in the experiments.

\subsection{Android Testing Tools}
Over the years, there have been many well-researched and developed automated Android testing tools.
In this study, we introduce four testing tools and frameworks in practice.
% \chen{I suggest to put this part backward to the evaluation section, as it is not our contribution. Just briefly introduce the overall principle of dynamic GUI testing here.}

\textbf{Monkey.}
~\cite{web:monkey} is a pure random testing tool, developed by Google. 
It emits pseudo-random streams of GUI events (e.g., touch, gestures) and some system events (e.g., volume controls, navigation).
% Monkey is widely-used in industry for automated testing because it is easy-to-use and compatible with any Android version.

\textbf{Ape.}
~\cite{gu2019practical} is a novel model-based GUI testing tool. 
It uses the run-time information to dynamically evolve its abstraction criterion via a decision tree to generate GUI events.

% It uses the run-time information to dynamically evolve its abstraction criterion via a decision tree, which can effectively balance the size and precision of the model. 
% Specifically, with this dynamically refined model, Ape generates GUI events via a random and greedy depth-first state exploration strategy. 
% Moreover, Ape also internally utilizes Monkey to occasionally emits random GUI events and system events to avoid stucking at local states.

\textbf{Droidbot.}
~\cite{li2017droidbot} is a versatile testing tool implemented in Python. 
It adopts several algorithms (e.g., greedy search, depth-first search, and breadth-first search) to dynamically construct an activity transition model on-the-fly and consume it to generate test events.
% Droidbot is fully implemented in Python, which allows a large variety of research and development.


\textbf{Humanoid.}
~\cite{li2019humanoid} is the first deep learning-based testing tool, built on DroidBot.
The underlying technique is a deep neural network that predicts which GUI elements are more likely to be interacted with by users and how to interact with them. 
% The model was trained upon a large-scale crowd-sourced human interactions dataset Rico~\cite{deka2017rico}. 
% It is expected to drive the GUI exploration towards important states faster as it prioritizes GUI elements according to their importance and meaningfulness like a human. 


\subsection{Configurations of Testing Tools}
Next, We explain some general configuration settings used in Android testing tools.

\textbf{$--$throttle.}
Throttle is to insert a fixed interval (milliseconds) between events for GUI transition to ensure testing on rendered GUI~\cite{sui2019event}.
% It is used to 
If the throttle value is set to 0, there is no interval, and the events are executed as rapidly as possible.
% \chen{Need to tell why GUI testing tool needs this.}
% In addition, a throttle event can create a fixed delay between other types of user events to allow the devices to process and react to the events just injected.

\textbf{$--$runtime.}
Runtime is the period of time when the testing is running. 
It begins when the first test event is sent and ends with the testing is done.

\textbf{$--$seed.}
Seed value specifies a particular stream from a set of possible pseudo-random number streams.
If you re-run the automated testing tools with the same seed value, it aims to generate the same sequence of events.
It is typically used to record and replay usage scenarios or bugs in testing.

\textbf{$--$ignore-crashes.}
Normally, the testing tool will stop when the app crashes or experiences any type of unhandled exception.
The option to ignore crashes is set to address this problem.
Once the app is detected to unexpectedly exit, the testing will automatically launch the app and continue to send events, until the allotted runtime is up.


==> results.tex <==
\section{Empirical Results}


\begin{table}
    \centering
	\caption{Performance comparison with baselines}
	\label{tab:rq1}
	\begin{tabular}{|l|c|c|}
	\hline
	\bf{Method} & \bf{Accuracy} & \bf{Inference Time} \\ 
	\hline
	SIFT-SVM & 0.757 & 15.81 ms\\
	SIFT-KNN & 0.635 & 1.20 ms\\
	SIFT-RF & 0.670 & 1.31 ms\\
	\hline
	SURF-SVM & 0.717 & 16.94 ms\\
	SURF-KNN & 0.631 & 1.27 ms\\
	SURF-RF & 0.670 & 1.29 ms\\
	\hline
	ORB-SVM & 0.706 & 18.10 ms\\
	ORB-KNN & 0.625 & 1.15 ms\\
	ORB-RF & 0.673 & 1.46 ms\\
	\hline
	CNN-FC & 0.841 & 18.10 ms \\
	ResNet-18 & 0.987 & 51.74 ms \\
	\hline
	\rowcolor{lightgray} \bf{Our Model} &  \bf{0.998} &  \bf{43.02 ms} \\
	\hline
	\end{tabular}
\end{table}

\begin{figure}
	\centering
	\subfigure[]{
		\includegraphics[width = 0.225\linewidth]{figures/bad_1.png}
		\label{fig:bad_1}}
	\hfill
	\subfigure[]{
		\includegraphics[width = 0.225\linewidth]{figures/bad_2.png}
		\label{fig:bad_2}}	
	\hfill
	\subfigure[]{
		\includegraphics[width = 0.225\linewidth]{figures/bad_3.png}
		\label{fig:bad_3}}	
	\hfill
	\subfigure[]{
		\includegraphics[width = 0.225\linewidth]{figures/bad_4.png}
		\label{fig:bad_4}}	
	\caption{: Examples of bad cases in GUI state prediction.}
	\label{fig:bad}
\end{figure}

\subsection{RQ1: Performance of Model}
Table~\ref{tab:rq1} depicts the accuracy and inference time for our model MobileNetV2 for classifying the fully rendered GUIs and partially rendered GUIs.
Our model achieves 99.8\% accuracy which is much higher than that of baselines, i.e., 31.8\% boost compared with the best machine learning baseline (SIFT-SVM).
Although the accuracy of our model and ResNet-18 are very similar, the inference time of our model is much faster, i.e., 8.72 milliseconds faster per GUI screenshot.
This indicates our model can accurately and efficiently discriminate the GUI rendering state.

Albeit the good performance of our model, we still make wrong prediction for some GUI screenshots. 
We manually check those wrong GUI cases, and summarise two common causes.
First, within some GUIs, the representative features are too tiny and inconspicuous to be recognized even with human eye, for example, the red linear progress bar in Figure~\ref{fig:bad_1}, and the tiny circular progress bar embedded in the image in Figure~\ref{fig:bad_2}.
Second, some negative data are not really negative data due to the different cognition of GUI state.
For example, since Figure~\ref{fig:bad_3} and \ref{fig:bad_4} are screenshots that contain dynamic assets such as videos and gifs, they are automatically annotated as partially rendered GUIs in temporal, while they seem to be fully rendered in spatial.


\begin{table*}
	\centering
	\footnotesize
	\caption{Performance comparison for our tool. "T" denotes the time to trigger the bug in seconds. "S" denotes whether the method successfully detect the bug.}
	\label{tab:rq2}
    \begin{tabular}{|l|r||c|c|c|c|c|c|c|c|c|c|c|c||c|c|c|c|} 
    \hline
        \multirow{2}{*}{\bf{Bug}} & \multirow{2}{*}{\bf{Step}} & \multicolumn{2}{c|}{\makecell{\bf{Throttle} \\ \bf{200ms}}} & \multicolumn{2}{c|}{\makecell{\bf{Throttle} \\ \bf{400ms}}} & \multicolumn{2}{c|}{\makecell{\bf{Throttle} \\ \bf{600ms}}} & \multicolumn{2}{c|}{\makecell{\bf{Throttle} \\ \bf{800ms}}} & \multicolumn{2}{c|}{\makecell{\bf{Throttle} \\ \bf{1000ms}}} & \multicolumn{2}{c||}{\bf{Themis}} & \multicolumn{2}{c|}{\makecell{\bf{Our Tool -}}} &  \multicolumn{2}{c|}{\cellcolor{lightgray} \bf{{Our Tool}}} \\
        \cline{3-18} &
        & T & S & T & S & T & S & T & S & T & S & T & S & T & S & \cellcolor{lightgray} T & \cellcolor{lightgray} S \\
    \hline
        \it{ActivityDiary\#118} & 10 & 12.77 & & 15.45 & & 17.31 & & 18.68 & & 20.54 & & 26.80 & & 17.56 & & \cellcolor{lightgray} 16.68 & \cellcolor{lightgray} \\
        
        \it{ActivityDiary\#285} & 10 & 13.99 & \xmark & 15.79 & & 17.22 & & 18.97 & & 21.31 & & 34.49 &  & 18.66 & & \cellcolor{lightgray} 15.80 & \cellcolor{lightgray} \\
        
        \it{AmazeFileManager\#1796} & 12 & 14.99 & & 17.03 & & 19.25 & & 21.49 & & 23.89 & & 51.46 & & 18.28 & & \cellcolor{lightgray} 17.63 & \cellcolor{lightgray} \\
        
        \it{AmazeFileManager\#1837} & 4 & 3.70 & & 4.21 & & 4.87 & & 5.40 & & 6.56 & & 10.41 & & 6.08 & & \cellcolor{lightgray} 5.48 & \cellcolor{lightgray} \\
        
        \it{and-bible\#261} & 18 & 20.31 & \xmark & 23.63 & \xmark & 27.29 & \xmark & 30.50 & \xmark & 33.88 & \xmark & 84.24 & & 28.60 & \xmark & \cellcolor{lightgray} 26.22 & \cellcolor{lightgray} \xmark \\
        
        \it{AnkiDroid\#4200} & 13 & 14.54 & \xmark & 16.90 & & 19.94 & & 22.29 & & 24.04 & & 28.91 & & 17.83 & & \cellcolor{lightgray} 16.86 & \cellcolor{lightgray} \\
        
        \it{AnkiDroid\#4451} & 19 & 23.42 &  & 26.77 & & 30.51 & & 34.08 & & 37.64 & & 39.52 & & 31.88 & & \cellcolor{lightgray} 29.61 & \cellcolor{lightgray} \\
        
        \it{AnkiDroid\#5638} & 4 & 3.58 & & 4.26 & & 4.85 & & 5.41 & & 6.01 & & 12.20 & & 4.97 & & \cellcolor{lightgray} 4.04 & \cellcolor{lightgray} \\
        
        \it{AnkiDroid\#5756} & 16 & 17.92 & \xmark & 21.04 & \xmark & 23.67 & \xmark & 26.67 &  & 29.76 &  & 34.91 & & 21.10 & & \cellcolor{lightgray} 20.73 & \cellcolor{lightgray} \\
        
        \it{AnkiDroid\#6145} & 24 & 38.20 & & 43.17 & & 48.08 & & 52.21 & & 56.94 & & 69.15 & & 46.05 &  & \cellcolor{lightgray} 39.77 & \cellcolor{lightgray} \\
        
        \it{APhotoManager\#116} & 3 & 2.39 & \xmark & 2.86 & \xmark & 3.22 & \xmark & 3.63 & \xmark & 4.07 & & 10.06 & & 2.88 & & \cellcolor{lightgray} 2.38 & \cellcolor{lightgray} \\
        
        \it{collect\#3222} & 9 & 9.49 & \xmark & 11.26 & \xmark & 12.74 & & 14.40 & & 16.00 & & 18.34 & & 11.85 & & \cellcolor{lightgray} 10.59 & \cellcolor{lightgray} \\
        
        \it{geohashdroid\#118} & 4 & 3.67 & \xmark & 4.18 & \xmark & 5.11 & \xmark & 5.40 & \xmark & 6.06 & \xmark & 12.49 & & 6.27 & \xmark & \cellcolor{lightgray} 5.70 & \cellcolor{lightgray} \xmark \\
        
        \it{Omni-Notes\#745} & 11 & 13.82 & & 15.79 & & 18.37 & & 19.57 & & 21.88 & & 28.94 & & 18.60 & & \cellcolor{lightgray} 17.36 & \cellcolor{lightgray} \\
        
        \it{open-event-attendee\#2198} & 5 & 5.19 & \xmark & 5.49 & \xmark & 6.30 & & 7.27 & & 8.09 & & 14.66 & & 6.59 & & \cellcolor{lightgray} 6.33 & \cellcolor{lightgray} \\
        
        \it{openlauncher\#67} & 4 & 5.21 & \xmark & 5.80 & & 6.38 & & 7.01 & & 7.61 & & 8.95 & & 5.76 & & \cellcolor{lightgray} 5.31 & \cellcolor{lightgray} \\
        
        \it{Scarlet-Notes\#114} & 23 & 27.92 & \xmark & 32.50 & & 37.06 & & 40.80 & & 45.87 & & 67.78 &  & 34.61 & & \cellcolor{lightgray} 30.10 & \cellcolor{lightgray} \\
        
        \it{WordPress\#10302} & 3 & 2.48 & & 2.87 & & 3.29 & & 3.67 & & 4.09 & & 10.25 & & 2.77 & & \cellcolor{lightgray} 2.32 & \cellcolor{lightgray} \\
        
    \hline
    \hline
    
    \it{Average} & 10.6 & 12.97 & 44\% & 14.94 & 66\% & 16.97 & 77\% & 18.75 & 83\% & 20.79 & 89\% & 31.31 & 100\% & 16.68 & 89\% & \cellcolor{lightgray} 15.16 & \cellcolor{lightgray} 89\% \\
    \hline
    \end{tabular}
\end{table*}


\subsection{RQ2: Performance of Tool}
Table~\ref{tab:rq2} shows detailed results of the time and success rate for each testing seed, where each app, and number of steps to detect the bug are displayed.
Our \tool successfully used an average of 15.16 seconds to successfully detect 89\% of the bugs.
Compared to our approach, the throttle methods of 200ms, 400ms, 600ms, 800ms, and 1000ms time delay, take on average 12.97, 14.94, 16.97, 18.75, and 20.79 seconds to detect the bugs, respectively.
The former three throttles only detect a few bugs than the latter two, especially throttle 200ms can only detect 44\% of the bugs.
In contrast, our tool can detect most of the bugs (89\%) in less time (15.16 seconds), that is detecting 23\% more bugs at similar runtime (e.g., Throttle 400ms), and increasing 27\% efficiency of same success rate (e.g., Throttle 1000ms).
Compared to our approach, the benchmark method Themis can detect 2 more bugs, but takes a relatively long time, on average 31.31 seconds, which is 2x slower than our approach.
This indicates that our approach can adaptively adjust the throttle delay between events, e.g., sending events to fully rendered GUI and explicitly waiting for partially rendered GUI, representing a balance between efficiency and effectiveness in testing.
In addition, leveraging real-time GUI rendering mointor accelerates the testing process than that of asynchronous mointor, saving 1.52 seconds for 10.6 steps on average.
As a result, much of time budget will be saved in hundreds or thousands steps of long-term testing.

We also manually observe the issues with our failure tests, and find one common reason.
Due to network latency, some GUIs require longer delay to load resources, which exceeds our maximum throttle limit ($>$ 1000ms).
Therefore, our approach continues to send the next event, which dispatches on an non-interactive GUI (e.g., loading page).
But we believe setting a longer maximum throttle threshold will potentially address the issue.








\begin{table}
    \centering
	\caption{Usefulness in real-world testing tool}
	\label{tab:rq3}
	\begin{tabular}{|l|c||c|c|c|}
	\hline
	\multirow{2}{*}{\bf{Method}} & \bf{Throttle} & \multirow{2}{*}{\bf{Coverage}} & \multicolumn{2}{c|}{\bf{GUI}} \\
	\cline{4-5}
	 & \bf{(ms)} &  & \bf{Number} & \bf{Quality} \\
	\hline
	\multirow{5}{*}{Droidbot} & 200 & 36.19\% & 2,832 & 77.48\% \\
	 & 400 & 34.47\% & 2,199 & 79.95\% \\
	 & 600 & 35.97\% & 1,501 & 83.75\% \\
	 & 800 & 35.11\% & 859 & 87.32\% \\
	 & 1000 & 30.15\% & 504 & \bf{91.67\%} \\
	\hline
	\rowcolor{lightgray} Droidbot+ &  adaptive & \bf{43.14\%} & \bf{3,207} & 88.81\% \\
	\hline
	\end{tabular}
\end{table}

\subsection{RQ3: Usefulness of Tool}
Table~\ref{tab:rq3} shows the results of the performance between Droidbot and our implement version of Droidbot+.
Droidbot+ achieves a median activity coverage of 43.14\% across 32 Android apps, which is 6.95\% higher even compared with the best baseline (e.g., 36.19\% in Throttle 200ms).
This is because the dynamic wait in Droidbot+ allows access to more activities that fast throttling might disrupt.
For example, while the GUI is in loading progress, a fixed throttle testing might send backward events to abandon exploration or random events to crash the application.
In addition, Droidbot+ explores 3,207 GUI states, and 88.81\% are fully rendered.
Compared to Droidbot+, the Droidbot throttled at 1000ms runs events on slightly higher quality GUIs (91.67\% vs 88.81\%), but it explores much slower (504 vs 3,207). 
This indicates the effectiveness and efficiency of our \tool in covering most of the activities and GUI states.



\begin{table}
    \centering
    \small
	\caption{\revise{Ablation study for our tool.} \chen{This is not ablation study. Why not put frame@5, or 15 as baselines to Table II?} \sidong{First, frame@n is a variant of our method, leveraging number of frames to single frame for rendering inference. Second, Table II is not wide enough to add frame@n or async results. I have made it clearer in writing.}}
	\label{tab:rq2_1}
	\begin{tabular}{l|c|c}
	\hline
	\bf{Method} & \bf{Time (T)} & \bf{ Reproducibility (R)} \\
	\hline
	Consecutive Frame@5 & 25.29 s & 83\% \\
	Consecutive Frame@15 & 33.57 s & 100\% \\
	Consecutive Frame@30 & 62.13 s & 100\% \\
	Asynchronous Streaming & 17.51 s & 100\% \\
	\hline
	\bf{Ours} & \bf{15.93 s} & \bf{100\%} \\
	\hline
	\end{tabular}
\end{table}
